Approximate Distributed Joins in Apache Spark

The join operation is a fundamental building block of parallel data processing. Unfortunately, it is very resource-intensive to compute an equi-join across massive datasets. The approximate computing paradigm allows users to trade accuracy and latency for expensive data processing operations. The equi-join operator is thus a natural candidate for optimization using approximation techniques. Although sampling-based approaches are widely used for approximation, sampling over joins is a compelling but challenging task regarding the output quality. Naive approaches, which perform joins over dataset samples, would not preserve statistical properties of the join output. To realize this potential, we interweave Bloom filter sketching and stratified sampling with the join computation in a new operator, ApproxJoin, that preserves the statistical properties of the join output. ApproxJoin leverages a Bloom filter to avoid shuffling non-joinable data items around the network and then applies stratified sampling to obtain a representative sample of the join output. Our analysis shows that ApproxJoin scales well and significantly reduces data movement, without sacrificing tight error bounds on the accuracy of the final results. We implemented ApproxJoin in Apache Spark and evaluated ApproxJoin using microbenchmarks and real-world case studies. The evaluation shows that ApproxJoin achieves a speedup of 6-9x over unmodified Spark-based joins with the same sampling rate. Furthermore, the speedup is accompanied by a significant reduction in the shuffled data volume, which is 5-82x less than unmodified Spark-based joins.

==> algorithms/algo-bloomfilter-joins-overview.tex <==
%\begin{center}		
\begin{algorithm}[t]

\myfontsize
\SetLine

{\commentfontsize
	
\if 0
/* Let $n$ be the number of input datasets, $|BF|$ be the bloom filter size and $fp$ is the false positive rate of the bloom filter */
\fi

// $n$: number of input datasets \\
// $|BF|$: size of the Bloom filter \\
// $fp$: false positive rate of the Bloom filter \\
// $R$: input datasets \\
}
$R = \{R_i\}, \forall i \in \{1, ..., n\}$\;

\underline{{\bf bloomFilterJoin}}($R$, $|BF|$, $fp$)

\Begin{
	   {\commentfontsize // {\em Build a bloom filter for  join input datasets}}\\
	   $bf$ $\leftarrow$ buildJoinFilter($R$, $|BF|$, $fp$)\;	   
       
	   {\commentfontsize // {\em Extract set of items that will participate in the join operation from $R$}}\\	   
	   $\forall i \in \{1... n\}$: $\bar{R}_i$ $\leftarrow$ BF.$filter(R_i)$\;

	   {\commentfontsize // {\em Perform approximation operation over $\bar{R}$}}\\
	   $result$ $\leftarrow$ $ \prod\limits_{1}^{n}\bar{R}_i$\;
	   \Return{result}
    }

\caption{\projecttitle's high-level operation. We first determine the data items that will participate in the join operation using our multi-way Bloom filter. We then remove the data items not participating in the join. Afterwards, we we perform approximation in the join via our novel sampling mechanism.}
\label{alg:bloomfilter-join-overview}
\end{algorithm}
	

==> algorithms/algo-multiway-bloomfilter-joins.tex <==
%\begin{center}		
\begin{algorithm}[t]

\myfontsize
\SetLine

\KwIn{
\\
$k$ sets of data items $inputs$\\
bloom filter size $bf\_size$ \\
bloom filter false positive rate $bf\_false\_rate$\\
}
%\textbf{Input}: $k$ sets of data items $inputs$\\
%bloom filter size $bf\_size$ \\
%bloom filter false positive rate $bf\_false\_rate$\\

{\commentfontsize // {\em Build a Bloom filter for the join input datasets}}\\
{\commentfontsize // {\em This function is executed at Driver}}\\
\textbf{Function} buildJoinFilter($inputs, bf\_size, bf\_false\_rate$) \\ { 
      \Begin{
            {\commentfontsize // {\em Create a new Bloom filter for the overlap between inputs }}\\
            $join\_bf$ $\leftarrow$ {\tt BloomFilter}($bf\_size$, $bf\_false\_rate$)\;
            \ForEach{$input$ in $inputs$} {
                {\commentfontsize // {\em Build a Bloom filter for all inputs}}\\
                 $bf$ $\leftarrow$ {\tt buildDatasetFilter}($input$, $bf\_size, bf\_false\_rate$)\;
                {\commentfontsize // {\em Merge dataset filters for the overlap between inputs }}\\
                 $join\_bf$ $\leftarrow$  $join\_bf$  {\tt AND} $bf$\;
            }
            \Return{$join\_bf$} 
        }
            %{\tt Broadcast}($joinl\_bf$)\;
            

{\commentfontsize // {\em Build a Bloom filter for an input dataset}}\\
\textbf{Function} buildDatasetFilter($input,  bf\_size, bf\_false\_rate$)\\ {
	\Begin{
        {\commentfontsize //{\em MAP PHASE: initialize a filter for each partition}}\\
        {
            $partition\_bf$ $\leftarrow$ {\tt BloomFilter}($bf\_size$, $bf\_false\_rate$)\; 
            \ForEach{$item$ in $input$} {
                $partition\_bf$.{\tt add}($item.key$)\;
        }        
        }

     
    	{\commentfontsize //{\em REDUCE PHASE: initialize a filter for combined partitions}}\\{
        $dataset_bf$ $\leftarrow$ {\tt BloomFilter}($bf\_size$, $bf\_false\_rate$)\;
        \ForEach{$partition\_bf$  from Map phase} {
        	{\commentfontsize // {\em Merge partition filters to the dataset filter}}\\
        	$dataset_bf$ $\leftarrow$ $bf$  {\tt OR} $partition\_bf$\;
        }
        \Return{$bf$}
        }
    }
 }

{\commentfontsize // {\em Perform bloom-filter based multi-way joins}}\\
{\commentfontsize // {\em This function is executed at Workers}}\\
\textbf{Function} bloomFilterJoin($inputs$, $join\_bf$) \\ { 
	\Begin{            
            $join\_inputs$ $\leftarrow$ $\emptyset$\;
             \ForEach{$input$ in $inputs$} {
             	  {\commentfontsize // {\em Extract items will participate the join operation}}\\
             	  $join\_input$ $\leftarrow$ $join\_bf$.{\tt Filter}($input$)\;
             	  $join\_inputs$.{\tt Append}($join\_input$)\;
             }
            
             {\commentfontsize // {\em Perform the join operation}}\\
             $join\_result$ $\leftarrow$ $\emptyset$\;
             \ForEach{$join\_input$ in $join\_inputs$} {
             	  $join\_result$  $\leftarrow$  $join\_result$.{\tt Join}($join\_input$)\; 
             }
         
             \Return{$join\_result$}            
    }
}
} 

\caption{\bf: Bloom filter based multi-way joins.}
\label{alg:bloom-filter-join-algo}
\end{algorithm}

==> approximation.tex <==
\section{Approximation in Distributed Joins}
\label{sec:approximation}

\input{figuresTex/fig-approxjoin-sampling.tex}

Unfortunately, in the case when the intersection fraction among input datasets is high, the above mechanism achieves negligible performance improvement: the overhead of the join is still the whole cross-product computation (see $\S$\ref{sec:evaluation}). To reduce this overhead, we further design a lightweight sampling mechanism to achieve low latency during joins by performing cross-product on only a subset of the data, while preserving the statistical properties of the full output.

% We describe this sampling mechanism in the next section.
% In this section, we present a sampling mechanism that performs stratified sampling over joins after the filtering stage.

In data analytics, the output of a join operation can contain data items with multiple different join keys.
If a simple random sampling on the output is performed, it is possible that some keys consisting of very few items are overlooked, worsening the
statistical quality of the sample.


{\em Stratified sampling}~\cite{stratified-sampling} overcomes this issue by ensuring that data items having different join keys can be fairly selected to represent the sample, and no join key will be overlooked. In stratified sampling, each distinct join key's data items are sampled independently with simple random sampling. As a result, the final sample will contain all join keys, preserving the statistical properties to represent the cross product.
% To preserve the statistical quality of input datasets, for each join key, this mechanism performs sampling (e.g., simple random sampling) over data items independently.

Consider an inner-join example of $J = R_{1} \Join R_2$, a pair $((k, v), (k', v'))$, where $(k, v) \in R_1$ and $(k', v') \in R_2$.
This produces a joined item $(k, (v, v') \in J$ if and only if $(k = k')$. For example, $R_1$ contains $(C_0, v_1)$, $(C_0, v_2)$, and $(C_0, v_3)$, and $R_2$ has $(C_0, v_4)$, $(C_0, v_5)$, $(C_0, v_6)$, and  $(C_0, v_7)$. The join operation based on key $C_0$ can be modeled as a complete bipartite graph (see Figure \ref{fig:approxjoin-sampling}). For stratified sampling over join, we perform random sampling on data items having the same join key (e.g., key $C_0$). This process therefore is equal to performing edge sampling on the complete bipartite graph (see figure \ref{fig:approxjoin-sampling}).

However, sampling edges from the complete bipartite graph would require building the graph, which would correspond to computing the full cross product. To avoid this cost, we propose a heuristic and describe its error.

Algorithm~\ref{alg:sampling-graph-algo} describes the algorithm with our heuristic to sample edges from the complete bipartite graph. To include an edge in the sample, we randomly select one endpoint node from each side and then yield the edge connecting these nodes. To obtain a sample of size $k$, we repeat this process $k$ times.

With this heuristic, the final sample can contain duplicate edges after the sampling, introducing some error on the sampled data. This error can be estimated via two alternatives.

% In addition, we can remove duplicate edges by using hash-based data structures such as HashTable or HashMap and repeat the algorithm steps until we reach the desired number of data items in the sample. However, this might worsen the randomness of the sampling mechanism, and so it could introduce bias in the sample data.  Fortunately, we can use a technique known as the Horvitz-Thompson~\cite{horvitz-thompson} estimator to easily remove the bias.

\input{algorithms/algo-sampling-graph.tex}

% \subsection{Error Estimation}
% \label{subsec:design-error-estimation}
% 
% %\myparagraph{False positive of bloom filter based joins} --> we added the modeling section for this
% 
% In \projecttitle, we need to handle the false positive rate introduced by bloom filters in the first stage and the accuracy loss introduced  by sampling in the second stage. For false positives, we build a model to analyze the trade-off between the shuffled data size with varying false positives (see $\S$~\ref{sec:modeling}). In this section, we describe how to compute the error bound estimation for the aggregate query results after the second stage --- stratified sampling process.

%\myparagraph{Error estimation for stratified sampling process} 
\myparagraph{Error estimation with the Central Limit Theorem}
We can use the Central Limit Theorem to estimate error bounds for the query output, because the sampling mechanism works as a random sampling with replacement. Suppose we want to compute the approximate sum of data items after the join operation. The output of the join operation contains data items with $n$ different keys $C_{1}$, $C_{2}$  $\cdots,$ $C_{n}$, each key (stratum) $C_{i}$ has $B_{i}$ data items and each such data item $j$ has an associated value  $v_{ij}$. To compute the approximate sum of the join output, we first select a sample of the join output data items based on the stratified sampling, i.e., we sample $b_{i}$ items from each join key $C_{i}$. Thereafter, we estimate the sum from this sample as $\hat{\tau} = \sum_{i=1}^{n} ( \frac{B_{i}}{b_{i}} \sum_{j=1}^{b_{i}}  v_{ij} ) \pm \epsilon$ 
where the error bound $\epsilon$ is defined as:
\begin{equation}\label{eq:epsilon}
\epsilon = t_{f,1-\frac{\alpha}{2}} \sqrt{\widehat{Var}(\hat{\tau})}
\end{equation}

Here, $t_{f,1-\frac{\alpha}{2}}$ is the value of the $t$-distribution (i.e., \textit{t-score}) with $f$ degrees of freedom and $\alpha = 1 - confidence level$. The degree of freedom $f$ is calculated as:
\begin{equation}\label{eq:degree_of_freedom}
f =  \sum_{i=1}^{n} b_{i} - n
\end{equation}

The estimated variance for the sum, $\widehat{Var}(\hat{\tau})$, can be expressed as:
\begin{equation}\label{eq:variance_sum}
\widehat{Var}(\hat{\tau}) = \sum\limits_{i=1}^n B_{i} * (B_{i} - b_{i}) \dfrac{r^2_{i}}{b_{i}}
\end{equation}

Here, $r^2_{i}$ is the population variance in the $i^{\textrm{th}}$ stratum. We use the statistical theories~\cite{samplingBySteve} for stratified sampling to calculate the error bound.

\myparagraph{Error estimation with the Horvitz-Thompson method}
One modification to the algorithm can be to avoid the duplicate edges by checking their presence in the already sampled data: when a duplicate edge is detected, we simply would sample the endpoint nodes again until another edge is yielded. This approach, however, would worsen the randomness of the sampling mechanism, introducing some bias to the sample. The Horvitz-Thompson estimator \cite{samplingBySteve} can be used to estimate this error.

Horvitz-Thompson is an unbiased estimator for the population sum and mean for any design of sampling, with or without replacement.
Let $\pi_i$ is a positive number representing the probability that data item having key $C_i$ is included in the sample under a given sampling scheme. Let $y_i$ is the sample sum of items having key $C_i$: $y_i = \sum_{j=1}^{b_{i}}  v_{ij}$. The Horvitz-Thompson estimation of the total is computed as~\cite{samplingBySteve}:

\begin{equation}\label{eq:sum-ht}
\hat{\tau_\pi}  = \sum_{i=1}^{n}( \frac{y_i}{\pi_i}) \pm \epsilon_{ht}
\end{equation}
where the error bound $\epsilon_{ht}$ is given by:
\begin{equation}\label{eq:epsilon-ht}
\epsilon_{ht} = t_{\frac{\alpha}{2}} \sqrt{\widehat{Var}(\hat{\tau_\pi})}
\end{equation}
where t has $n - 1$ degrees freedom. The estimated variance of the Horvitz-Thompson estimation is computed as:
\begin{equation}\label{eq:variance_sum-ht}
\widehat{Var}(\hat{\tau_\pi}) = \sum\limits_{i=1}^n (\frac{1 - \pi_i}{\pi_{i}^{2}})*y_i^{2} + \sum\limits_{i=1}^n \sum\limits_{j \neq i}^{} (\frac{\pi_{ij} - \pi_{i}\pi_{j}}{\pi_{i}\pi_{j}}) * \frac{y_{i}y_{j}}{\pi_{ij}}
\end{equation}
where $\pi_{ij}$ is the probability that both data items having  key $C_i$ and $C_j$ are included.
The Horvitz-Thompson estimation does not depend on how many times a data item may be selected. Each distinct item of the sample is used only once~\cite{samplingBySteve}. 




==> background.tex <==
\subsection{Distributed Joins in Big Data Systems}
\label{sec:background}

%\pramod{\bf Explain the join mechanisms in Apache Spark/Hadoop/Flink. We should rewrite focusing NOT on the different types of joins, BUT we should highlight how joins are implemented in Big Data Systems.}
%\input{figuresTex/fig-join-mechanisms-comparison.tex}
%\input{figuresTex/fig-bf-overlap-fractions.tex}

%\input{figuresTex/fig-join-mechanisms-background.tex}

Many big data systems, such as Apache Spark~\cite{spark}, Apache Flink~\cite{flink} and Hadoop~\cite{hadoop}, partition the input datasets into smaller data chunks stored on different nodes of a deployment cluster. Although this partitioning helps with storing and processing large datasets in a fault-tolerant and parallel fashion, it also creates a challenge for join operations involving multiple datasets: the join operation requires the systems to move data items from one node to another, so that the cross-product operation can be performed on each node. To perform this data movement, the systems typically adopt two join strategies: {\em (i)} repartition join and {\em (ii)} broadcast join.


%Most big data systems have adopted a data parallel programming model {\em MapReduce} to handle massive input data~\cite{mapreduce-join,spark-nsdi-2012,hadoop}.  




%\todo{shorten and fix}
%\projecttitle adopts {\em data flow} computing model for distributed and parallel join operations. In the data flow programming model, an application is presented as a data-dependency graph. Each vertex in this graph represents an operation and each edge presents the communication between operations (vertices). The operations are isolated from each other and executed when inputs are available. Operations which share no data dependency among them can be executed concurrently. This programming model is well-adopted in big data systems~\cite{spark, flink} to explore parallelism in distributed environments.
%In this section, we give an overview and explain the shuffle data issue of join processing mechanisms in a distributed environment, especially in Apache Spark. 

%\subsection{Map-side Join}
%Map-side joins make use of a mechanism that is similar to sort-merge joins in traditional database systems. This approach executes join operation by performing a cross-product at the map side and requires no shuffle/reduce phase~\cite{mapreduce-join}. The disadvantage of this mechanism is that it requires the input datasets to be split into the same number of partitions using the same hash function, so that the data items having the same keys will end up on the same machine. In addition, it cannot handle data skew where a partition contains many data items having the same join key. Thus, the machine storing this partition could quickly run out of memory during the map-side join process.

\myparagraph{Repartition Join}
\label{subsec:repartition-join}
This mechanism is the default join execution approach in big data systems~\cite{spark, flink, sparkbook}. The basic idea is to ensure that data items having the same join keys from all input datasets are collected at the same node in the cluster. To achieve this goal, the input datasets are repartitioned using the same partitioner (e.g., the same hash function), so that a given join key is collected by a single node. This node then performs the cross-product operation between the data items.  

The advantage of this mechanism is that it does not require sophisticated steps to perform the join operation: The repartitioning operation can be modeled as a simple MapReduce job, whose shuffle phase naturally transfers the data items to the desired nodes. The disadvantage, however, is that this transfer can involve a significant amount of data and the transferred data items can include items that are not going to participate in the join. When the overlap fraction of the data items in different datasets is low, this approach leads to significant overhead in data transfer, which can also affect latency (see Section \ref{sec:evaluation}).

\myparagraph{Broadcast Join}
\label{subsec:broadcast-join}
When one input dataset is much smaller than the others, the systems can broadcast the smaller dataset to all nodes storing the other datasets. Afterwards, the join operation is performed at the map phase of the processing~\cite{mapreduce-join}.
Broadcast join is very efficient for joins between a single, large dataset and one or more small datasets, because it avoids moving the data items of the large dataset through the network. However, this situation may not always be possible in real world traces (see $\S$\ref{sec:case-studies}).

%Figure~\ref{fig:join-mechanism} (a) illustrates an example of the repartition join. After the repartitioning process, all items with even keys will be transferred to node $0$, and all items with odd keys will end up on node $1$.

%The advantage of this mechanism is that it fits naturally into the MapReduce model and does not require sophisticated steps to perform the join operation. The disadvantage of this approach is that it requires the shuffle phase of the MapReduce job to transfer data items through the cluster. The transferred data items can include items that are not going to participate in the join (e.g., items with keys $3$, $6$, and $8$ in Figure~\ref{fig:join-mechanism} (a)). When the overlap fraction of the data items in different datasets is low, this approach leads to significant overhead in data transfer, which can also affect latency (see Section \ref{sec:evaluation}.


%As the name implies this mechanism performs join operations at the reduce side~\cite{mapreduce-join} after repartitioning the inputs. At the map phase, the mechanism maps input join keys to associate values. Thereafter, it shuffles these immediate key/value pairs to the corresponding reducers using a hash function, i.e., the items with the same join key will end up at the same node in the cluster. At the reduce phase, it performs the cross-product operation for pairs having the same join key. Figure~\ref{fig:join-mechanism} (b) shows an example of the repartition join. After the repartitioning process, all items with even keys will end up at node $0$, and all items with odd keys will end up and node $1$.  The disadvantage of this approach is that it requires the shuffle phase to shift data items through the cluster including non-join items (items with keys $3$, $6$, and $8$)

%\myparagraph{Broadcast Join}
%\label{subsec:broadcast-join}
%When one input dataset is much smaller than the others, the systems can broadcast the smaller dataset to all other nodes hosting the other datasets instead of moving all input datasets across the network. Afterwards, the systems perform the join operations at the map phase of the processing~\cite{mapreduce-join}.
%
%Figure~\ref{fig:join-mechanism} (b) shows an example. The dataset $R$ contains only two data items. As a result, it is broadcast from node $0$ to all other nodes (e.g., node $1$). These other nodes then perform the cross product operation.
%
%Broadcast join is very efficient for joins between a single, large dataset with one or more small datasets because it avoids moving the data items of the large dataset through the network. However, this situation may not always be possible in real world traces (see $\S$\ref{sec:case-studies}). %\iea{is this really the case in the real world datasets we have?}

%This mechanism is used the when one input dataset is much smaller than the others. Instead of moving all input datasets across the network, this mechanism simply sends the smaller dataset to all nodes containing the other datasets (see Figure~\ref{fig:join-mechanism} (a)). Thereafter, it performs the join operations at the map phase~\cite{mapreduce-join}. Figure~\ref{fig:join-mechanism} (a) shows that since the input dataset $R$ contains only two data items, the mechanism broadcasts it from node $0$ to all nodes in the cluster (node $1$) and then performs the cross-product operation in each node. 


%When one input dataset is much smaller than the other, instead of moving all input datasets across the network, this mechanism simply sends the smaller dataset to all nodes containing the other dataset (see Figure~\ref{fig:join-mechanism} (a)). Thereafter, it performs the join operations at the map phase~\cite{mapreduce-join}. Figure~\ref{fig:join-mechanism} (a) shows that since the input dataset $R$ contains only two data items, the mechanism broadcasts it from node $0$ to all nodes in the cluster (node $1$) and then performs the cross-product operation in each node.
%This mechanism reduces the amount of shuffled data over the network compared to repartition join (see $\S$~\ref{subsec:repartition-join}) since it does not require the input repartition using the same hash function as repartition join. However, it requires the size of one input dataset to be small enough to broadcast to all nodes involved in join operations. In the case that the size of input datasets is larger, this approach incurs significant shuffled data  as shown by Figure~\ref{fig:join-mechanism-comparison} (a). The simulation-based experiment (see $\S$~\ref{sec:modeling}) shows the total shuffled data size with different join mechanisms. 



\if 0
\subsection{Bloom Filter Based Two-Way Join}
This mechanism improves the performance of repartition join by avoiding sending non-participating data items in join operations through the network (see Figure~\ref{fig:join-mechanism} (c)). It filters out items from an input dataset where their join keys are not matching with other keys from other input datasets (items with keys $3$, $6$, and $8$). This approach makes use of a {\em bloom filter} - a space-efficient data structure to eliminate the non-participating data items~\cite{bloomfilter-join}. In the case the overlap fraction between input datasets (or the selectivity of the join operation) is small, this mechanism significantly reduce the shuffled data size as highlighted in Figure~\ref{fig:join-mechanism-comparison} (a).

However,  the disadvantage of this approach is that It require extra computations to build the filter by scanning entire the input datasets. In addition, when the overlap fraction or the selectivity of the join operation is high, the mechanism does not significantly reduce the shuffled data (see Figure~\ref{fig:join-mechanism-comparison} (b)). The simulation result shows that with the overlap fraction of $80\%$, the bloom filter based join produces a similar shuffled data size with the repartition join mechanism.
Moreover, the bloom filter based join achieves little/no performance gains in terms of latency since the main overhead of the join operation comes from the cross-product process.

To overcome the problem of bloom filter based join mechanism, we propose \projecttitle which adds one more stage beside the filtering stage to gracefully handle the overhead of join operations. %using approximate computing.
\fi


==> benchmarks.tex <==
%\subsection{Micro-benchmarks}
%\label{subsec:microbenchmarks}
%
%\input{figuresTex/fig-benchmark-error}
%\input{figuresTex/fig-num-answers-error}
%\input{figuresTex/fig-fraction-yes-error}
%\input{figuresTex/fig-splitx-comparison}
%
%We first conducted micro-benchmarks to analyze the impact of the sampling and randomizing parameter selection on the utility and the user privacy (see $\S$~\ref{subsubsec:sampling-randomizing}), as well as the impact of the number of participated {\em Clients} and the fraction of origin truthful `yes' answers on the utility. Then, to measure the overhead of crypto operations of \projecttitle and previous systems, we built micro-benchmarks on a laptop, a smartphone and a high-performance server. Finally, we conducted an experiments with 2 cluster nodes to measure latency of components in our system with a previous system, that has a similar architecture with our system, namely {\em SplitX}~\cite{Chen-2013}. Each result of experiments is generated after 100 independent runs.
%%a MacBook Air laptop with a 2,2 GHz Intel Core i7 CPU, 8GB of RAM running OS X Yonsemite as well as on a smartphone with a 1 GHz CPU running Android 4.1.2.
%
%\subsubsection{ What is the effect of varying sampling and randomizing parameters $r$, $p$ and $q$?}
%\label{subsubsec:sampling-randomizing}
%We study the effect of sampling and randomizing parameters on the utility and user privacy by applying our sampling and randomizing mechanism to  synthetic datasets. For this experiment, we first randomly generate $10,000$ original answers with 80\% of them are 'yes`. Then, we measure the utility and the privacy with different values of the parameters by using the equation~\ref{thrm:zkp} and equation~\ref{eq:accuracyloss}, respectively.
%
%Figure \ref{fig:benchmark-error} depicts the utility with different values of the sampling and randomizing parameters, whereas Figure~\ref{fig:case-study-privacy} represents the privacy with various values of the sampling and randomizing parameters. The smaller accuracy loss $\eta$ means higher utility, and smaller privacy level $\epsilon$ means stronger privacy. The sampling and randomizing parameters handle the trade-off between the utility and the privacy guarantee of the query results. 
%
%To analyze the effect of the randomizing parameters $p$ and $q$ on the utility and the privacy guarantee, the sampling parameter is set to $60$\%. The results of this experiment are presented  on the table \ref{tab:utility-privacy}. When $p$ and $q$ are set with a smaller value, the system provides stronger privacy for use but achieves lower utility e.g., with $p = 0.3$ and $q = 0.3$,  $\epsilon = 1.7047$ and $\eta = 0.245$, whereas when $p$ and $q$ are set with a bigger value, the system provides higher utility but weaker privacy e.g., with $p = 0.9$ and $q = 0.9$,  $\epsilon = 3.1570$ and  $\eta = 0.0594$.
%
%
%\begin{table}[t!]
%\small
%\centering
%\begin{tabular}{c|c|c|c}
%\hline $p$ & $q$ & Accuracy loss ($\eta$) & Privacy Level ($\epsilon$) \\
%\hline
%\hline \multirow{3}{*}{0.3} & 0.3 & 0.2450 & 1.7047\\
%  & 0.6 & 0.2128 & 1.3862\\
%  & 0.9 & 0.1530 & 1.2527\\
%\hline \multirow{3}{*}{0.6} & 0.3 & 0.1154 & 2.5649\\
%  & 0.6 & 0.0986 & 2.0476\\
%  & 0.9 & 0.0902 & 1.7917\\
%\hline \multirow{3}{*}{0.9} & 0.3 & 0.0730 & 4.1820 \\
%  & 0.6 & 0.0682 & 3.5263\\
%  & 0.9 & 0.0594 & 3.1570\\
%\hline
%\end{tabular}
%\vspace{-2mm}
%\caption{The utility and the privacy guarantee of query results with different randomizing $p$ and $q$. The utility is measured by the query result's relative error (see expression~\ref{eq:accuracyloss}), and privacy is calculated by the level of achieved zero-knowledge privacy (see expression~\ref{eq:ezk}).  The number of original answers is set to $10,000$ with $80$\% of them are `yes'. The sampling parameter $r$ is set to $0.6$. Each result is generated after 100 independent runs.}
%\vspace{-2.5mm}
%\label{tab:utility-privacy}
%\end{table}
%
%\subsubsection{What is the effect of varying numbers of participated {\em Clients} on the utility?}
%Next, we analyze the impact of different numbers of participated {\em Clients} on the utility with constant sampling and randomizing parameters. For this experiment, we keep sampling and randomizing parameters--fixed. In detail, $p$, $q$ and $r$ are set to $0.9$ and the fraction of original answers are `yes' is fixed to $80$\%. Figure~\ref{fig:num-answers-error} depicts the effect of varying numbers of {\em Clients} on the utility. The result of this experiment shows that the processing answers of too few participated {\em Clients} could lead to very low utility (i.e., very high accuracy loss) of the query results.
%
%\subsubsection{What is the effect of varying fractions of origin truthful `yes' answers on the utility?}
%In the next experiment, we evaluate the impact of varying fractions of origin truthful `yes' answers on the utility. We measure the utility with different fractions of original truthful `yes' answers, meanwhile keep other parameters--sampling, randomizing parameters, and the total number of original answers--fixed. The number of original answers is set to $10,000$ and the sampling and randomizing parameters $p$, $q$ and $r$ are set to $0.9$. Figure~\ref{fig:num-answers-error} represents the experiment results. The system achieves higher utility as the fraction of original truthful `yes' answers increases. This is because of the randomized response mechanism. If the fraction of truthful answers being `yes' is high, then the utility of the query results generated based on randomized answers of {\em Clients} will be also high.
%
%\subsubsection{What is the encryption computation overhead compared to previous systems?}
%In privacy-preserving analytics systems, crypto operations are used to provide stronger privacy guarantees to users. However, the overhead of crypto operations is a major bottleneck of the system. Therefore, we conduct experiments to measure the computation overhead of \projecttitle and previous systems~\cite{RSA, Chen-2012, Paillier}. The crypto operations of previous system are RSA~\cite{RSA}, Goldwasser-Micali~\cite{Chen-2012}, and Paillier~\cite{Paillier}; whereas the crypto operations of \projecttitle is XOR operations.
%Note that, the Paillier-based approach~\cite{Paillier} is not resistant to the pollution attacks. Even a single malicious {\em Client} can substantially distort the query results in the Paillier-based system without any detection. Although the Paillier-based approach contains this weakness, we still want to add it in these experiments for the computation overhead comparison.
%
%We analyzed the computation overhead of crypto methods on various types of devices: 1) Android Galaxy mini III smartphone running Android 4.1.2 with a 1.5 GHz CPU, 2) MacBook Air laptop with a 2,2 GHz Intel Core i7 CPU, 8GB of RAM running OS X Yonsemite 10.10.2. 3) Linux server running Linux 3.15.0 with a 2.2 GHz CPU with 32 cores. In particular, we measured the number of cryto operations can be executed on each device per second. Table~\ref{tab:overhead} shows, not surprisingly, that the XOR operation of \projecttitle are extremely efficient compared to crypto methods of previous systems. In other words,  the XOR operations will not create any significant performance bottleneck in \projecttitle.
%
%
%\begin{table*}[t!]
%\small
%\centering
%\begin{tabular}{r|r|r|r|r|r|r}
%\hline
%                                                                           & \multicolumn{3}{c|}{Encryption}      & \multicolumn{3}{c}{Decryption}                \\ \hline 
%                                                                           & Phone    &  Laptop     & Server         & Phone          & Laptop          & Server \\ \hline \hline
%RSA in~\cite{RSA}           & 937      &   2,770       & 4,909         & 126            & 698              & 859              \\ \hline
%Goldwasser in~\cite{Chen-2012}   & 2,106    &  17,064    & 22,902        & 127            & 6,329           & 7,068           \\ \hline
%Paillier in~\cite{Paillier}     & 116       &  489         & 579             & 72              & 250              & 309              \\ \hline
%XOR in \projecttitle                                               & 15,026  &  943,902  & 1,351,937   & 3,262,186  & 16,519,076  & 22,678,285   \\ \hline
%\end{tabular}
%\vspace{-2mm}
%\caption{Computational overhead of cryptographic operations (\# operations / second).  The public-key crypto schemes use a 1024-bit key.}
%\vspace{-9mm}
%
%\label{tab:overhead}
%\end{table*}
%
%\subsubsection{What is the latency at {\em Proxies} compared to the previous system {\em SplitX}?}
%A previous system~\cite{Chen-2013}, namely {\em SplitX}, is also able to defeat the pollution attacks and contains similar components as \projecttitle. However, unlike \projecttitle, {\em SplitX} requires synchronization among system components to apply the randomized response mechanism to query answers at {\em Proxies} (in {\em SplitX}, the {\em Proxies} components are called {\em Mixes}). The synchronization creates a significant delay in processing query answers, and this prevents the usage of {\em SplitX} for stream analytics. We conducted experiments to measure the latency at {\em Mixes} of {\em SplitX} as well as {\em Proxies} of \projecttitle in processing query answers. Figure~\ref{fig:splitx-comparison} depicts the latency comparison in processing query answers at {\em Proxies} between {\em SplitX} and \projecttitle with different numbers of participated {\em Clients}. The log-log plot shows a not surprising result that the latency at {\em Mixes} of {\em Splitx} is significant higher than the latency at {\em Proxies} of \projecttitle. With $1,000,000$ {\em Clients}, the latency at {\em SplitX} is $40.276\ seconds$, while this value of \projecttitle is $6.209\ seconds$.
%  
%Figure~\ref{fig:case-splitx-comparison} depicts the latency comparison between {\em Mixes} (Splitx) and {\em Proxies} (PrivApprox).


==> building-blocks.tex <==
\section{Building Blocks}
\label{subsec:buildingblocks}
Before describing in detail the design of the \projecttitle, we introduce the techniques we used in that design in this section.



\subsection{Differential Privacy} 
\pramod{Martin: Do we need a background on zero-knowledge privacy and how it compares with differential privacy?}

Differential privacy~\cite{differential-privacy} has become  the standard privacy mechanism which protects the privacy of individual inputs in a statistical database by ensuring that the output of any analysis on the database is not influenced considerably by the existence of any individual input. A computation $C$ gives $\varepsilon-$differential privacy if for all datasets $D_1$ and $D_2$ differing on at most one record (i.e. one input), and all output $O \subseteq Range(C)$:

\begin{equation}
\label{eq:differential-privacy}
 Pr[C(D_1) \in O] \leq e^{\varepsilon} \times Pr[C(D_2) \in O]
\end{equation}

The probability of a computation $C$ produces a given output is almost independent of the existence of any individual input in the dataset. In other words,  the output distribution of a computation changes very little when one individual input is added or removed from the dataset. As a result, it makes very difficult to determine whether or not  an individual input is in the dataset, therefore protecting privacy of the individual input.
The privacy parameter $ \varepsilon$ controls the accuracy/privacy tradeoff. Smaller $ \varepsilon$ provides stronger privacy but lower accuracy and vice versa.



\subsection{Randomized Response}
\label{subsec:randomizing}

\pramod{Martin could you please make a careful pass}
To provide the differential privacy property, a randomized  process is need. A popular mechanism for the randomized process is randomized response, that allows individuals to not provide truthful answers all the time to sensitive queries, but still provide statistical results to analysts. Suppose that an analyst send a query to individuals to obtain statistical data about a sensitive property $P$. Each individual randomizes its answer to the query as follows. The individual flips a coin, if it comes heads, then respond truthful answers, otherwise the individual flips a second coin and response ``Yes'' if it comes heads and `No' if it comes tails. The privacy is guaranteed via the ability to refuse responding truthful answers of individuals. 

Suppose that the probability of the first coin and second coin coming up heads are $p$ and $q$, respectively. If the analyst receives $N$ randomized answers from individuals, and $Ry$ answers in the randomized answers are ``Yes'', then the number of original truthful ``Yes'' answers before the randomizing process is estimated as follows:

\begin{equation}
\label{eq:estimatedAnswer}
E_y = \dfrac{R_y - (1- p)\times q \times N}{p} 
\end{equation}

Suppose $A_y$ and $E_y$  are the actual and the estimated number of the original truthful ``Yes'' answers, respectively. The accuracy loss $\eta$ is defined as follows:
 
 \begin{equation}
\label{eq:accuracyloss}
\eta = \abs{ \dfrac{A_y - E_y}{A_y} }
\end{equation}
 
From~\eqref{differential-privacy}, we have that the randomized response mechanism achieve $\varepsilon-$ differential privacy, with:

\begin{equation}
\label{eq:privacy-level1}
\varepsilon = ln(\dfrac{Pr[Response = ``Yes'' | Truth = ``Yes'']}{Pr[Response = ``Yes'' | Truth = ``No'']} )
\end{equation}

If a truthful answer is ``Yes'', then the probability of the randomized answer will be still ``Yes'', is $p + (1 - p) \times q$. In addition, if a truthful answer is `No', then the probability of the randomized answer will be still ``Yes'', is $(1 - p) \times q$. Therefore:

\begin{equation}
\label{eq:privacy-level2}
\varepsilon = ln(\dfrac{p + (1 - p) \times q}{(1 - p) \times q})
\end{equation}


%\subsection{Query Buckets}
%\projecttitle supports SQL languages for {\em analysts} to create queries to {\em clients} (see details in $\S$~\ref{sec:design}). The range of query answer values is divided into buckets, i.e., each bucket represent a small range of query answer values. Each query answer is represented in the form of binary buckets, where each bucket stores a possible answer value `1' or `0' depending on whether or not the answer falls into the value range represented by that bucket. 
%For example, to get the nationality distribution among students in a university, e.g. {\em TU Berlin}, an analyst can create a SQL like {\em ''SELECT nationality FROM students WHERE university = `TU Berlin'}. The range of possible answer values is split into four buckets `Europe', 'Americas', 'Asia', and 'Africa'. If a given student comes from Brazil, the client answers `1' for the second bucket and `0' for all remaining buckets. Although answering the queries with the bit buckets is quite simple at first glance, it has been indicated to be effective in a large number of statistical analytics algorithms~\cite{statistical-analysis}.

\subsection{One-Time Pad (OTP) Encryption}
\label{subsec:otp}
\input{figuresTex/fig-otp-encryption.tex}

To achieve high performance, \projecttitle uses One-Time Pad (OTP) for message encryption, which has been previously proposed in the context of anonymous communication~\cite{ anonymity12, Chen-2012, Chen-2013}. At a high-level, OTP employs extremely efficient bitwise XOR operations as its cryptographic primitive compared to expensive public-key cryptography. 


The underlying idea of OTP is quite simple:  If Alice wants to send a secret message $M$ to Bob, then  Alice and Bob share a secret one-time pad $K$ (in the form of a random bit-string of length $l$). To transmit the message, Alice first converts $M$ into the form of bit-string of length $l$, and sends a encrypted message $M' = M \oplus K$ to Bob, where $\oplus$ denotes the bit-wise XOR operation. To decrypt the message,  Bob uses the bit-wise XOR operation: $M = M' \oplus K$.


 %Figure~\ref{fig:queryans} represents the use of OTP in \projecttitle to answer queries (see $\S$~\ref{sec:answerqueries}).

Figure~\ref{fig:otp} shows how the OTP-based encryption is used to transmit messages from a {\em client} to the {\em aggregator} via two {\em proxies}. The client transmits the message $M$ to the {\em aggregator} as follows. First, the client generates a random $l$-bitstring $M_K$ using a cryptographic pseudo-random number generator (PRNG) seeded with a cryptographically strong random number. Next, it performs an XOR operation with $M$ and $M_K$ to produce an encoded message $M_E$.
 
\begin{equation}
M_E = M \oplus M_K
\end{equation}


After that, the client sends  $M_E$  with a message identifier $M_{ID}$ to the first proxy, and $M_K$ with  $M_{ID}$ to the second proxy.  The message identifier  $M_{ID}$ is a unique large random number generated by the client. The {\em aggregator} receives the messages and joins them using the message identifier $M_{ID}$. The {\em aggregator} then recreates the original message $M$ by performing the XOR operation on $M_E$ and $M_K$.

 \begin{equation}
M = M_E \oplus M_K
\end{equation}

This OTP mechanism allows {\em clients} to anonymously transmit query answers to the {\em aggregator} via {\em proxies} (see $\S$~\ref{sec:answerqueries}).


%\pramod{please add a figure, and necessary text to explain it properly. See SplitX paper for the same.} 


\subsection{Approximate Computation}
\label{subsec:approx}
 By relaxing the need for exact results, approximation computation allows us to achieve low latency and efficient resources  utilization by computing over a partial subset in stead of the entire input datasets. Given this advantage,  several approximate computing mechanisms have been proposed~\cite{BlinkDB,approxhadoop} for ``Big Data'' analytics. In \projecttitle, we applied a input data sampling mechanism for approximate computation.

\myparagraph{Simple random sampling (SRS)}  
Simple random sampling is the most basic sampling technique where a subset of units (a sample) is selected from a population of units for study. Each individual in the population has the same chance of being included in the sample.  
In \projecttitle, we make the use of SRS at the {\em clients} to select participated clients. SRS is performed at the {\em clients} as follows. Each client flips a coin, and it will decide to participate answering a query base on whether or not the coin comes head (see $\S$~\ref{sec:answerqueries}).

Suppose that we have a population of $U$ clients; each client $i$ has an associated answering value $a_i$; and we want to calculate the sum of these values across the population $\sum\limits_{i}^{U} a_i $. To compute an approximate sum, we apply the SRS at {\em clients} to get a sample of $U'$ clients. The estimated sum is calculated as follows:

\begin{equation}
\hat{\tau} = \dfrac{U}{U'}\sum\limits_{i}^{U'} a_i  \pm \epsilon
\end{equation}

where the error bound  $\epsilon$ defined as:
 
\begin{equation}
\label{eq:epsilon}
\epsilon = t\sqrt{\widehat{Var}(\hat{\tau})}
\end{equation}

Note that the $t$ in the equation for the bound is a value of the Student t-distribution with $U' - 1$ degrees of freedom at the $1 - \alpha/2$ level of significance.
and the estimated variance of sum is represented as:

\begin{equation}\label{eq:variance_sum}
\widehat{Var}(\hat{\tau}) = \dfrac{U^2}{U'}s^2(\dfrac{U -  U'}{U})
\end{equation}

where $s^2$ is the variance of sum.


==> design.tex <==

%\input{figuresTex/fig-system-overview.tex}
%\input{figuresTex/fig-dataflow}

In this section, we present our approach built in \projecttitle to reduce overhead of join operations in big data analytics.
\subsection{System Model}
 Before we present the detailed design of \projecttitle, we describe the system model used in this work.
\projecttitle adopts {\em data flow} computing model for distributed and parallel join operations. In the data flow programming model, an application is presented as a data-dependency graph. Each vertex in this graph represents an operation and each edge presents the communication between operations (vertices). The operations are isolated from each other and executed when inputs are available. Operations which share no data dependency among them can be executed concurrently. This programming model is well-adopted in big data systems~\cite{spark, flink} to explore parallelism in distributed environments.


\subsection{System Workflow}
Figure \ref{fig:system-overview} represents the high-level design of \projecttitle.
Suppose we want to compute an equal-join on attribute $A$ for $n$ input datasets $R_1 \Join R_2 \Join ... \Join R_n$, where $R_i (i = 1, ..., n)$ is an input dataset. For simplicity, we assume that $n = 2$. 

To proceed the join operation, we first build a join bloom filter (see $\S$~\ref{subsec:design-bloomfilter}) which is a probabilistic data structure representing the intersection of the input datasets.
Next, we use this filter to eliminate data items not participating in the join operation.
Thereafter, we perform sampling (detailed in $\S$~\ref{subsec:design-sampling}).
The sampling algorithm ensures that the joined data items are randomly selected and none of the join keys are excluded, thereby preserving the statistical quality of the input datasets. 

The operations after the join process on the sampled data and provide an approximate result to users together with an error bound in the form of $output \pm error bound$.
Since our sampling mechanism preserves randomness, we can use the error estimation mechanism based on the Central Limit Theorem~\cite{samplingBySteve} to compute the error bounds (see $\S$~\ref{subsec:design-error-estimation}).


Unfortunately, in the case when the intersection fraction among input datasets is high, the above mechanism achieves negligible performance improvement, since the overhead of the join is still the whole cross-product computation (see $\S$\ref{sec:evaluation}). To reduce this overhead, we further design a light-weight sampling mechanism to achieve low latency during joins by performing cross-product on only a subset of the data. We describe this sampling mechanism in the next section.




==> figuresTex/fig-bf-implementation.tex <==
\begin{figure}[t]
\centering
\includegraphics[scale=0.26]{figuresTex/figures/bf-implementation.png}
\caption{Distributed Dataflow graph of multi-way Bloom filter building.}
%\caption{The implementation of join bloom filter module using Apache Spark}
\label{fig:bf-implementation}
\end{figure}


==> figuresTex/fig-bf-overlap-fractions.tex <==
\begin{figure}[t]
    \centering
    \includegraphics [width=0.42\textwidth]{figuresTex/figures/bf-overlap-shufflesize.eps} 
    \caption{The shuffled data size of repartition join and bloom filter based join with different overlap fractions  (Simulation with 100 nodes cluster and with 3 input datasets) }
     %\vspace{-5mm}
\label{fig:join-bf-overlap-fractions}
\end{figure}

==> figuresTex/fig-bloomfilter-size.tex <==
\begin{figure}[t]
\centering
\includegraphics [width=0.42\textwidth]{figuresTex/figures/bloom-filter-size.eps}
\caption{The latency and the data shuffle size of \projecttitle  in the join processing}
%\vspace{-5mm}
\label{fig:bloomfilter-size}
\end{figure}


==> figuresTex/fig-case-studies.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics [width= 1\textwidth]{figuresTex/figures/case-studies.eps} 
    \caption{\textbf{(a)} The latency and the shuffled data size of \projecttitle w/o sampling and Spark join systems in network traffic case study; \textbf{(b)} The latency comparison between \projecttitle w/ sampling and Spark repartition join w/ sampling before join operation in network traffic case study ; \textbf{(c)} the accuracy loss of \projecttitle and Spark repartition join w/ sampling before join operation with varying overlap fractions in network traffic case study; \textbf{(d)} the latency of \projecttitle, Spark repartition join w/sampling after join operation, and native Spark join in Netflix case study. }
     %\vspace{-5mm}
\label{fig:case-studies}
\end{figure*}

==> figuresTex/fig-case-study-netflix.tex <==
\begin{figure}[t]
\centering
\includegraphics [width=0.45\textwidth]{figuresTex/figures/case-study-netflix.eps}
\caption{ Comparison between  \projecttitle and Spark join systems in Netflix case study: \textbf{(a)}  Latency and shuffle data; \textbf{(b)} Latency with various sampling fractions.}
%\vspace{-5mm}
\label{fig:case-study-netflix}
\end{figure}

==> figuresTex/fig-case-study-network-accuracy.tex <==
\begin{figure}[t]
\centering
\includegraphics [width=0.42\textwidth]{figuresTex/figures/case-study-network-accuracy.eps}
\caption{The accuracy comparison between \projecttitle, Spark joins w/ sampling}
%\vspace{-5mm}
\label{fig:case-study-network-accuracy}
\end{figure}

==> figuresTex/fig-case-study-network.tex <==
\begin{figure*}[t]
\centering
\includegraphics [width=1\textwidth]{figuresTex/figures/case-study-network.eps}
\caption{ Comparison between  \projecttitle and Spark join systems in network traffic case study: \textbf{(a)}  Latency and shuffle data; \textbf{(b)} Latency with various sampling fractions; \textbf{(c)} Accuracy loss with various sampling fraction.}
%\vspace{-5mm}
\label{fig:case-study-network}
\end{figure*}

==> figuresTex/fig-dataflow-implementation.tex <==
\begin{figure}[t]
\centering
\includegraphics[scale=0.24]{figuresTex/figures/dataflow-implementation.png}
\caption{Distributed Dataflow graph \projecttitle.}
\label{fig:dataflow-implementation}
\end{figure}


==> figuresTex/fig-dataflow.tex <==
\begin{figure}[t]
\centering
\includegraphics[scale=0.33]{figuresTex/figures/dataflow-model.png}
\caption{Data flow programming model}
\label{fig:dataflow-model}
\end{figure}

==> figuresTex/fig-error-microbenchmark.tex <==
\begin{figure}[t]
\centering
\includegraphics [width=0.42\textwidth]{figuresTex/figures/error-microbenchmark.eps}
\caption{The accuracy loss comparison between \projecttitle with sampling and Spark-based joins with varying sampling fractions}
%\vspace{-5mm}
\label{fig:error-microbenchmark}
\end{figure}


==> figuresTex/fig-implementation-new.tex <==
\begin{figure}[t]
\centering
\includegraphics[scale=0.2]{figuresTex/figures/approxjoin-implementation.png}
\caption{Distributed Dataflow graph of \projecttitle.}
\label{fig:approxjoin-implementation}
\end{figure}


==> figuresTex/fig-implementation.tex <==
\begin{figure}[t]
\centering
\includegraphics[scale=0.3]{figuresTex/figures/implementation-new}
\caption{Architecture of \projecttitle prototype (shaded boxes depict the implemented modules)}
\label{fig:system-implementation}
\end{figure}


==> figuresTex/fig-join-mechanisms-comparison.tex <==
\begin{figure}[t]
    \centering
   % \includegraphics [width=0.42\textwidth]{figuresTex/figures/shuffle-overlap.eps}
    \includegraphics [width=0.42\textwidth]{figuresTex/figures/join-mechanisms-comparison.eps} 
    \caption{The shuffled data size comparison between join mechanisms (Simulation with 100 nodes cluster, the overlap fraction between input datasets is set to $1\%$) }
     %\vspace{-5mm}
\label{fig:join-mechanism-comparison}
\end{figure}

==> figuresTex/fig-join-mechanisms.tex <==
\begin{figure*}[t]
\centering
\includegraphics [width=1\textwidth]{figuresTex/figures/join-mechanisms}
\caption{Distributed join mechanisms}
\vspace{-5mm}
\label{fig:join-mechanism}
\end{figure*}


==> figuresTex/fig-latency-netflix.tex <==
\begin{figure}[t]
\centering
\includegraphics [width=0.42\textwidth]{figuresTex/figures/latency-netflix.eps}
\caption{The latency comparison between  \projecttitle, Spark repartition join, and native Spark join with various sampling fractions.}
%\vspace{-5mm}
\label{fig:latency-netflix}
\end{figure}

==> figuresTex/fig-latency-overlap.tex <==
\begin{figure*}[t]
\centering
\includegraphics [width=1\textwidth]{figuresTex/figures/latency-overlap.eps}
\caption{The latency comparison between \projecttitle without sampling and Spark-based joins}
\vspace{-5mm}
\label{fig:latency-overlap}
\end{figure*}


==> figuresTex/fig-latency-sampling.tex <==
\begin{figure}[t]
\centering
\includegraphics [width=0.42\textwidth]{figuresTex/figures/latency-sampling.eps}
\caption{The latency comparison between \projecttitle with sampling and Spark-based joins with varying sampling fractions}
%\vspace{-5mm}
\label{fig:latency-sampling}
\end{figure}


==> figuresTex/fig-multiway-joins.tex <==
\begin{figure}[t]
\centering
\includegraphics [width=0.42\textwidth]{figuresTex/figures/multiway-join-comparison.eps}
\caption{The latency and data shuffle size comparison  between \projecttitle without sampling and Spark-based joins with various number of input datasets.}
%\vspace{-5mm}
\label{fig:multiway-joins}
\end{figure}


==> figuresTex/fig-multiway-latency-overlap.tex <==
\begin{figure}[t]
\centering
\includegraphics [width=0.42\textwidth]{figuresTex/figures/multiway-latency-overlap.eps}
\caption{The multi-way join processing latency comparison between \projecttitle without sampling and Spark-based joins}
%\vspace{-5mm}
\label{fig:multiway-latency-overlap}
\end{figure}

==> figuresTex/fig-multiway-shuffle-overlap.tex <==
\begin{figure}[t]
\centering
\includegraphics [width=0.42\textwidth]{figuresTex/figures/multiway-shuffle-overlap.eps}
\caption{The data shuffle size comparison  between \projecttitle without sampling and Spark-based joins in the multi-way join processing}
%\vspace{-5mm}
\label{fig:multiway-shuffle-overlap}
\end{figure}


==> figuresTex/fig-scalability.tex <==
\begin{figure}[t]
\centering
\includegraphics [width=0.42\textwidth]{figuresTex/figures/latency-scalability.eps}
\caption{The latency comparison between \projecttitle, Spark repartition join, and native Spark join with different number of nodes in the cluster}
%\vspace{-5mm}
\label{fig:scalability}
\end{figure}

==> figuresTex/fig-shuffle-overlap.tex <==
\begin{figure}[t]
\centering
\includegraphics [width=0.42\textwidth]{figuresTex/figures/shuffle-overlap.eps}
\caption{The data shuffle size comparison between \projecttitle without sampling and Spark-based joins}
%\vspace{-5mm}
\label{fig:shuffle-overlap}
\end{figure}


==> figuresTex/fig-tpch-10g-sampling-accuracy.tex <==
\begin{figure}[t]
\centering
\includegraphics [width=0.42\textwidth]{figuresTex/figures/snappy-approxjoin-tpch-10G-accuracy.eps}
\caption{The latency comparison between \projecttitle and SnappyData with different sampling fractions}
%\vspace{-5mm}
\label{fig:tpch-10g-sampling-accuracy}
\end{figure}


==> figuresTex/fig-tpch-10g-sampling-latency.tex <==
\begin{figure}[t]
\centering
\includegraphics [width=0.42\textwidth]{figuresTex/figures/snappy-approxjoin-tpch-10G-latency.eps}
\caption{The latency comparison between \projecttitle and SnappyData with different sampling fractions}
%\vspace{-5mm}
\label{fig:tpch-10g-sampling-latency}
\end{figure}


==> figuresTex/fig-tpch-10g.tex <==
\begin{figure}[t]
\centering
\includegraphics [width=0.42\textwidth]{figuresTex/figures/tpc-h-10g.eps}
\caption{The latency and the data shuffle size of \projecttitle  in processing TPC-H queries}
%\vspace{-5mm}
\label{fig:tpch-10g}
\end{figure}


==> problem-statement.tex <==
\subsection{Problem Statement}
\label{subsec:problem-statement}

\input{figuresTex/fig-sampling-join-comparison.tex}


%\pramod{\bf I: Explain the cost of join operation (using empirical measurements), and how it becomes worse with increasing data sizes / and number of tables. Also, give a teaser of what approxjoins can achieve here.}
%
%\pramod{\bf II: Motivate the approximation mechanism to overcome this problems, talk about the possible interfaces for approximation (latency/accuracy trade-off)}
%
%\pramod{\bf III: Define formally the problem statement (with Greek letters), and also mention the input/output to the overall approach. Basically explaining the interface of the system but formally/}

Join operations are often considered critical in big data systems. Unfortunately, they are expensive operations even with the state-of-the-art big data systems, such as Apache Spark and Apache Flink. This high cost is not only related to the computation but also to the communication required to performed the join operation. In practice, these big data systems can take hours or even days to process a join operation between dataset that is gigabytes or terabytes in size.

A na\"ive solution to improve the performance of joins is to employ more computing resources, which comes at a significant monetary cost. An alternative approach is to utilize approximate computing, where only a subset of input data is used to obtain results. Approximate computing trades off accuracy for low latency and efficient resource utilization, by providing users with approximate results with associated error bounds. In the case of joins of big datasets, this trade-off is based on the observation that the exact results of a distributed join operation may not be necessary: the computation of exact results incurs additional delay for user response, but does not provide any additional value. 

One widely used technique for approximate computing is sampling. Sampling over joins, however, is not a straightforward task and becomes challenging, especially in a distributed environment. One approach -- {\em  pre-join sampling} -- performs sampling over the input datasets before the join and uses the samples to perform the join operation. Although this approach is simple and quite fast, it produces poor quality output, as explained in $\S$~\ref{sec:introduction} (see Figure~\ref{fig:sampling-join-comparison} (a)). Another approach -- {\em post-join sampling} -- preserves the statistical properties of the join output by performing sampling after the join operation is finished. Unfortunately, this sampling requires the entire join operation to complete, and thus, introduces significantly high latency (see Figure~\ref{fig:sampling-join-comparison} (b)). 

A recent join approach, Wander Join \cite{wander-join}, aims to model the join relationship among the data items as a graph, where a vertex represents a data item and an edge is drawn between two vertices if they can join with each other. Wander Join then performs {\em random walks}, so that each path would correspond to a sampled join output. However, Wander Join is not designed for distributed settings. It also does not consider non-participating keys in the join operation, so that `null' results can occur in the output.

We make the following observations: Distributed analytics systems deal with a huge amount of data. The latency and accuracy of join operations in these systems become sensitive to the amount of data transferred during the join; therefore, it is important to ensure that only necessary data items are transferred over the network. Furthermore, the size of the input datasets also means that the cross product phase in the join operation can have a detrimental effect on the latency for obtaining the join results.

\myparagraph{The case for approximation in distributed joins} 
Filtering data items not participating in the join can reduce the amount of data transfer significantly; thus, reducing the latency of the join operation. However, this reduction depends on the number of such data items: if the `overlapping fraction' (i.e., data items that are going to participate in the join) is large, these items will still have to be transferred over the network. More importantly, the bottleneck of the join operation will shift to the cross product of these items (see \S\ref{sec:evaluation}). Figure~\ref{fig:join-mechanism-comparison} (b) also shows that even with a relatively small overlap fraction value of $40$\%, the amount of transferred data is comparable with the repartition join mechanism.

%In addition, these non-join data items may incur significant overhead for the shuffle stage of the join operation since the join mechanisms, that are widely used in big data systems (see $\S$\ref{sec:background}), do not distinguish data items that are not participating in the join operation. As a result, they end up redundantly transferring significant amounts of data over the network for the non-join data items. 
%
%To solve this problem, we introduce a filtering stage (see $\S$\ref{sec:bloom_multiway}) that filters out non-join items before the join operation, and thus, avoids transferring them through the network.



%We make two observations about the join mechanisms that are widely used in big data systems. Our first observation is that these systems incur significant overhead for the shuffle stage of the join operation. This overhead is due to the fact that these systems do not distinguish data items that are not participating in the join operation when they are preparing the dataset partitions. As a result, they end up redundantly transferring significant amounts of data over the network for the non-join data items. 

%This problem is only exacerbated when there are more than two datasets participating in the join operation. According to our simulations, Figure~\ref{fig:join-mechanism-comparison} (a) shows that the shuffled data size increases gradually with the number of datasets involved in the join operation. Even though the broadcast join seems to incur less overhead than the default repartition join, it requires that at least one dataset is small enough to be broadcast. In cases where multiple datasets are of similar size, the broadcast join cannot sustain the same performance.

%Compared with these approaches, an approach that can filter non-join items before the join operation can avoid the redundant data transfer. For example, a Bloom filter based join operation can filter data items whose join keys in the datasets do not match (e.g., items with keys $3$, $6$, and $8$ in Figure~\ref{fig:join-mechanism} (a)). Figure~\ref{fig:join-mechanism-comparison} (a) also shows that this approach can still significantly reduce the amount of data transferred, even when the number of datasets in the join operation increases.

%While broadcast join and repartition join mechanisms are widely used in the most big data systems, they incur the shuffle stage which introduces an overhead in the performance of join operations. In addition, the overhead will get even bigger when more input datasets is added in the join operation. Figure~\ref{fig:join-mechanism-comparison} (a) shows that the shuffled data size gradually increases with the increasing the number of input datasets. Here, the total data shuffled size during join operations is computed using a simulation-based experiment (see $\S$~\ref{sec:modeling}).
%Compare to repartition join, the broadcast join mechanism may reduce the amount of shuffled data over the network since it does not require the input repartition using the same hash function as repartition join. However, it requires the size of one input dataset to be small enough to broadcast to all nodes involved in join operations. In the case that the size of input datasets is larger, this approach incurs significant shuffled data  as shown by Figure~\ref{fig:join-mechanism-comparison} (a). 

%%{BRING THIS TO 3.1}Although one could think that reducing the amount of transferred data by filtering the non-join data items is sufficient to improve performance of distributed join operations, it is not a silver bullet: In cases where the overlap fraction between input datasets (i.e., the selectivity of the join operation) is high, this mechanism still has to transfer a large number of data items over the network for the join operation. Figure~\ref{fig:join-mechanism-comparison} (b) shows that even with a relatively small overlap fraction value of 40\%, the amount of transferred data in the shuffle stage is comparable with the repartition join mechanism. As a result, the join operation can still incur a significant computation overhead during the cross-product phase.



%To improve the performance of broadcast join and repartition join, we propose a filtering mechanism implemented in \projecttitle to avoid sending non-join data items through the network (see Figure~\ref{fig:join-mechanism} (c)). This filtering mechanism filters out items from an input dataset where their join keys are not matching with other keys from other input datasets (items with keys $3$, $6$, and $8$). In the case the overlap fraction between input datasets (or the selectivity of the join operation) is small, this mechanism significantly reduces the shuffled data size as highlighted in Figure~\ref{fig:join-mechanism-comparison} (a). However, when the overlap fraction or the selectivity of the join operation is high, the mechanism does not significantly reduce the shuffled data (see Figure~\ref{fig:join-mechanism-comparison} (b)). The simulation result shows that with the overlap fraction of $80\%$, the bloom filter based join produces a similar shuffled data size with the repartition join mechanism. Thus, the filtering approach achieves little/no performance gains in terms of latency since beside the shuffling overhead, broadcast join and repartition join mechanisms also need to suffer the main overhead comes from the cross-product process.
%
%To  handle the overhead of the cross-product process, a straightforward solution is to employ more computing resources for the big data systems. However, it comes at a higher computing cost.  To achieve both low-latency and efficient resource utilization in executing the cross-product process of join operations, we make use of approximate computing. This computing paradigm computes over a subset of input data instead of the whole input data, thus it can reduce the latency and computing resources. We apply approximate computing in \projecttitle by employing a sampling-based approach for taking samples over joins. The computation after joins is performed on the sampled data to provide an approximate result with an associate error bound to users. 

%Next, we provide an analysis of the latency of distributed joins in big data systems.
%Formally, we observe that the latency of the distributed join operations is a function of (i) the data transferred during the shuffle phase of the join computation and (ii) the cross product computation. Let $d_{dt}$ and $d_{cp}$ represent the delay associated with the data transfer during the shuffle phase and the delay with the cross product, respectively. 
%
%Generally speaking, the total delay for the join operation, $d_{join}$, would be:
%\begin{equation}
%d_{join} = d_{dt} + d_{cp} + d_{other}
%\end{equation}
%where $d_{other}$ represents other operations related to the coordination of the above events. There is significant research on how to minimize the overhead for the coordination of big data systems \cite{}. For the purposes of this paper, we assume that $d_{other}$ is negligible. Therefore, we can rewrite the above equation as:
%\begin{equation}
%d_{join} = d_{dt} + d_{cp}
%\label{eqn:delay-join}
%\end{equation}


% \projecttitle  allows users to trade-off the output quality (i.e., query accuracy) ) for low-latency and efficient resource utilization by providing a simple interface. The system interface induces {\em(i)} a query --- where users define the computation they want to execute on the sampled data and {\em {ii}} a budget --- where users define their desired latency or desired error bound requirements.
%\projecttitle needs to identify an optimal sample size for the sampling process based on the budget to ensure the query is executed within the budget.

%Assume that a user send a query $q$ and a query budget  $q_{budget} = \{l_{desired}, err_{desired}\}$ to our system; where $l_{desired}$ is the desired latency, and $err_{desired}$ is the desired error bound. \projecttitle uses a cost function $cost\_f$ to convert the budget into the sampling parameter: $sampleSize = cost\_f(q_{budget})$.  Next, the system takes a sample over the join operation with the sample size $sampleSize$: $sample = sample\_f(sampleSize)$, then it executes the query $q$ on the sample to provide the user an approximate result $approx$ with associate error bound $e\_bound$:
%
%\begin{equation}
%\label{eq:approxjoin-query}
%approx, e\_bound = query\_f(sample)
%\end{equation}

% In general, the end-end latency of \projecttitle is computed as follows:
%
%\begin{equation}
%\label{eq:approxjoin-latency}
%\begin{split}
%l_{total} = &\quad l_{filtering} +  l_{computing\_sampleSize} + l_{sampling} + \\
%              &\quad + l_{cross-product} +  l_{query}
%\end{split}
%\end{equation}
%
%Where $l_{filtering}$ is the latency of the filtering process,  $l_{computing\_sampleSize}$  is the processing time to compute the sample size, $l_{sampling}$ is the latency of the sampling process, $l_{cross-product}$ is the latency of the cross product process, and  $l_{query}$ is the latency of the query processing.

%The cost function needs to make sure to provide an optimal sample size $sampleSize$ such as: $e\_bound \leq err_{desired}$ and $l_{total} \leq l_{desired}$.

